ASR-Generated Text for Language Model Pre-training Applied to Speech Tasks

We aim at improving spoken language modeling (LM) using very large amount of automatically transcribed speech. We leverage the INA (French National Audiovisual Institute) collection and obtain 19GB of text after applying ASR on 350,000 hours of diverse TV shows. From this, spoken language models are trained either by fine-tuning an existing LM (FlauBERT) or through training a LM from scratch. New models (FlauBERT-Oral) are shared with the community and evaluated for 3 downstream tasks: spoken language understanding, classification of TV shows and speech syntactic parsing. Results show that FlauBERT-Oral can be beneficial compared to its initial FlauBERT version demonstrating that, despite its inherent noisy nature, ASR-generated text can be used to build spoken language models.

==> (Interspeech) Training a Language Model from ASR-generated Text for Spoken Language Understanding/downstream_syntax.tex <==
%\textbf{[TODO: reduce as well !]}

In this section, the downstream task consists in jointly predicting part of speech tags (POS) and building a labelled dependency tree from speech transcripts.
%The models performing these tasks typically rely on word representations, that are often pretrained, especially when the data is scarce.
We use our different LMs to generate contextual word representations and use them for predicting syntactic parses of speech transcripts.
%For each of these representations, a model is trained to perform  joint prediction of POS tags and labelled dependencies.
We contrast the obtained results to a baseline model trained using FastText non-contextual representations,\footnote{\url{https://fasttext.cc}} and a model learning its own representations without any pretraining.

\subsection{The ORFEO dataset}

Our study relies on the annotated subset of the speech corpus of the ORFEO project \cite{benzitoun2016projet, nasr:hal-02973242}, gathered with the goal of reflecting the contemporary usage of the French language.
The audio recordings include work meetings, family dinners, narrations, political meetings, interviews, and goal-oriented telephone conversations.
Their duration varies from 4mn to 1h. 
%minutes to an hour.
%Reference audio transcripts have been obtained after correcting the output of an ASR system.
%has been automatically transcribed then manually corrected.
The corpus is annotated with part-of-speech (POS) tags, lemmas, labeled dependency trees and sentences boundaries.
Annotations include 20 possible POS tags and 12 syntactic functions.
We randomly split the corpus into train/dev/test sets of respective sizes 134,716/27,937/29,529 words; we sampled from each source so that the various genres of speech are equally represented in each split.

\subsection{Parsing Model}

The syntax-predicting model is a transition based parser using the arc-eager transition system, which has been extended for the joint prediction of POS tags and parsing transitions \cite{dary-nasr-2021-reading}.
A single classifier is trained to predict transitions from features extracted from the current state of the analysis (word embebdings, predicted tags, history of transitions), for stack elements and a sliding window of size [-3;2] centered on the current word.
The POS sequence and dependency trees are greedily built from the sequence of transitions predicted by the classifier.
%The output of the classifier is a probability distribution over either POS tags or arc-eager labelled transitions, that will greedily determine the next action to take.
A dropout of 50\% is applied to the input vector, which passes through two hidden layers of size 3200 and 1600, both with 40\% of dropout and ReLU activations. The two decision layers are linear with a softmax.
Training runs for 40 epochs, using a dynamical oracle \cite{goldberg2012dynamic}, with scoring against the development set to select the best checkpoint.

\subsection{Experiments}

The first set of experiments compares input representations from the FlauBERT variants (FBU, FT, MIX, ORAL) to  non-contextual baselines. As with other experiments, LMs are applied on uncased transcripts without punctuation, which is not fair to the FBU model as it expects punctuation. Therefore we add a contrastive system with periods added at the end of each utterance prior to applying the LM (called FBU repunc), but added tokens are not passed to the parser, they just inform other embeddings.
Note that except for random initialized embeddings, token representations are not fine-tuned during training.
%not finetuned in a similar fashion to probing experiments, the rest of the model weights are learned.

As pre-processing, we deanonymize the transcripts by replacing masked proper name tokens with non-ambiguous names randomly chosen for each recording. In the fasttext setting, representations are computed for unknown words from their character n-gram factors. Token representations are computed at the whole recording level in chunks of 512 tokens without overlap. The parser is applied on the reference transcript and reference segmentation. We use mean pooling for words that are split in multiple tokens by BPE.

Parsing performance is evaluated with Labeled Attachment Score (LAS), the accuracy of predicting the governor of each word and its dependency label, Unlabeled Attachment Score (UAS), which ignores dependency labels, and Part-of-speech tagging accuracy (UPOS) (scoring script from CoNLL campaigns).

Results presented in Table~\ref{t:syntax-main} show that pre-training is valuable for syntactic parsing in that setting and that pretraining on ASR-generated text (\textbf{FT}, \textbf{MIX} and \textbf{ORAL}) leads to a substantial improvement in LAS over the text-only FlauBERT model (\textbf{FBU}) even though there is no domain overlap between the TV shows on which the LMs are trained and the data of the ORFEO corpus. As in the previous task, we see no benefit in retraining BPEs (\textbf{ORAL\_NB}). Performance in the \textbf{FBU repunc} settings is on par with the best model, showing that absence of punctuation is an important factor affecting performance when applying text-only models, at least for predicting syntax. 

\begin{comment}
\begin{table}[htb]
\centering
\begin{tabular}{lrrr}
\hline
\bf Repr. &	\bf LAS &	\bf UAS &	\bf UPOS \\
\hline
No pretraining & 	84.92 &	88.48 &	94.51 \\
Fasttext &	85.36 &	88.76 &	95.12 \\
\hline
FBU &	85.55 &	89.02 &	93.36 \\
\hline
FT &	86.81 &	90.22 &	95.01 \\
MIX	& 86.33	& 89.79	& 94.43 \\
ORAL	& \bf 87.65	& \bf 90.92	& 95.55 \\
ORAL\_NB & 87.54	& 90.73 & \bf 95.63 \\
\hline
\end{tabular}
\caption{Syntax prediction task: metrics are Labeled Attachment Score (LAS), Unlabeled Attachment Score (UAS) and Part-of-speech tagging accuracy (UPOS). Higher is better.}
\label{t:syntax-main}
\end{table}
\end{comment}

\begin{table}[htb]
\centering
\caption{Syntax prediction task: metrics are Labeled Attachment Score (LAS), Unlabeled Attachment Score (UAS) and Part-of-speech tagging accuracy (UPOS). Higher is better.}
\begin{tabular}{@{}lccc@{}}
\toprule
\bf Model &	\bf LAS &	\bf UAS &	\bf UPOS \\
\midrule
No pretrain & 	$84.92 \pm 0.44$ &	$88.48 \pm 0.37$ &	$94.51 \pm 0.29$ \\
Fasttext &	$85.36 \pm 0.10$ &	$88.76 \pm 0.05$ &	$95.12 \pm 0.03$ \\
\midrule
FBU &	$85.55 \pm 0.05$ &	$89.02 \pm 0.16$ &	$93.36 \pm 0.06$ \\
FBU repunc	& $87.48 \pm 0.28$	& $90.69 \pm 0.19$	& $95.03 \pm 0.03$ \\
\midrule
FT &	$86.81 \pm 0.09$ &	$90.22 \pm 0.06$ &	$94.99 \pm 0.10$ \\
MIX	& $86.33	\pm 0.15$ & $89.79	\pm 0.05$ & $94.43 \pm 0.29$ \\
ORAL	&  $\textbf{87.65}	\pm 0.11$ &  $\textbf{90.92}	\pm 0.10$ & $95.55 \pm 0.04$ \\
ORAL\_NB & $87.54 \pm 0.11$	& $90.73 \pm 0.08$ &  $\textbf{95.63} \pm 0.05$ \\
\bottomrule
\end{tabular}
\label{t:syntax-main}
\end{table}


%It is interesting to note that the MIX model is not as good as the ASR model although it contains ASR transcripts.

%\begin{table}[htb]
%centering
%\begin{tabular}{llrrr}
%\hline		
%\bf Repr. & \bf Context &	\bf LAS	& \bf UAS &	\bf UPOS \\
%\hline
%FBU & Conversation	& 85.55	& 89.02	& 93.36 \\
%FBU & Turn	& 74.17	& 80.20	& 80.60 \\
%FBU & Sentence	& 70.63	& 76.65	& 77.97 \\
%\hline
%\end{tabular}
%\caption{Effect of context when computing representations for syntactic parsing. Results for the FBU model when representations are extracted with different context. Similar trends are observed for the other models. Note that the FBU model was trained at the sentence level.}
%\label{t:syntax-context}
%\end{table}

%The original FlauBERT model is trained one sentence at a time with rather long sentences. Sentences of less than 20 tokens are stripped prior to training. The concept of sentence is less well-defined for speech than text, and it is frequent to see very short utterances which correspond to single tokens such as yes-no answers, backchannels, etc. As outlined in Table~\ref{t:syntax-context}, the choice of context is crucial for obtaining good performance on syntactic parsing. Interestingly, even though the FBU model has not been trained with full documents as context, it performs clearly better if a large context is accounted for. The typical independence between sentences assumption of syntaxic parsing would lead to very poor parsing performance, probably due to the fact that the model has not seen short sentences in training. 

\begin{comment}
\begin{table}[htb]
\centering
\begin{tabular}{@{}lccc@{}}
\toprule			
\bf Model & \bf LAS	& \bf UAS	& \bf UPOS \\
%\hline
%FBU	& 85.55	& 89.02	& 93.36 \\
%FBU w/ punct	& 87.48	& 90.69	& 95.03 \\
%\hline
%ORAL	& 87.65	& 90.92	& 95.55 \\
\midrule
FBU &	$85.55 \pm 0.05$ &	$89.02 \pm 0.16$ &	$93.36 \pm 0.06$ \\
FBU repunc	& $87.48 \pm 0.28$	& $90.69 \pm 0.19$	& $95.03 \pm 0.03$ \\
\midrule
ORAL	&  ${87.65}	\pm 0.11$ &  ${90.92}	\pm 0.10$ & $95.55 \pm 0.04$ \\
%ORAL	& 87.65	& 90.92	& 95.55 \\
\bottomrule
\end{tabular}
\caption{Effect of repunctuating speech transcripts on syntactic parsing prior to extracting representations. Results from the ORAL representations are given for reference.}
\label{t:syntax-punct}
\end{table}
\end{comment}

%As noted earlier, speech recordings do not have punctuation and it is debated whether punctuation is suitable for spontaneous conversations. As punctuation is rather regular in text, it would make sense for LMs trained on text to over-rely on the cues it brings, and representations to be affected by a lack of punctuation. Table~\ref{t:syntax-punct} shows syntactic parsing results on representations where a simple heuristic is applied to add a period at the end of each sentence prior to extracting representations. This punctuation is stripped before passing the tokens to the syntactic parser and only used at the encoding stage. Results show that most of the difference in performance between the \textbf{FBU} and \textbf{ORAL} models can be compensated by this use of virtual punctuation. Using accurately predicted punctuation with diverse symbols and intra-sentence marks is left as future work, but we conjecture that it will marginally improve over this crude heuristic.

\begin{comment}


\begin{table*}[htb]
\centering
\begin{tabular}{l|rrr|rrr|rrr}
\hline										
\bf Repr.	& \multicolumn{3}{c|}{\bf LAS}			& \multicolumn{3}{c|}{\bf UAS}			& \multicolumn{3}{c}{\bf UPOS}	 \\	
	& Global	& OOV	& $\Delta$	& Global	& OOV	& $\Delta$	& Global	& OOV	& $\Delta$ \\
\hline
FBU	& 85.55	& 74.10	& -11.45	& 89.02	& 82.20	& -6.82	& 93.36	& 79.00	& -14.36 \\
MIX	& 86.33	& 74.40	& -11.93	& 89.79	& 82.47	& -7.33	& 94.43	& 80.35	& -14.07 \\
ORAL	& 87.65	& 73.68	& -13.97	& 90.92	& 82.81	& -8.11	& 95.55	& 79.00	& -16.55 \\
\hline
\end{tabular}
\caption{Syntactic parsing performance on OOV words according to automatic transcription system. The $\Delta$ column contains the difference between the global accuracy and the accuracy on OOVs only.}
\label{t:syntax-oov}
\end{table*}

Gauging the impact of speech-to-text errors on representations from LMs trained on such data is difficult since there are no manual references available for large quantities of speech transcripts. Since the system used to transcribe the recordings is closed vocabulary, one way to look at this problem is to compute the accuracy of the syntactic parser on words that are out-of-vocabulary (OOV) for the LM training data. Due to BPE, those words are necessarily tokenized in smaller units which are pooled prior to passing them to the parser, and might affect the quality of the associated representations. Table~\ref{t:syntax-oov} details the performance of the syntactic parser on OOVs. Due to their infrequent nature, OOVs are mainly swear words, proper names, and tokenization artifacts. They are difficult to handle for all models, and suffer from a large performance reduction compared to the global figure, even for the \textbf{FBU} model which has seen a much larger variety of texts. The system fed with  representations of the model trained on ASR data only (\textbf{ORAL}) is the most affected despite its better global performance.

%Franck: On peut retirer la learning curve pour gagner un peu de place

\begin{figure}[htb]
\centering
\includegraphics[width=.9\linewidth]{plots/LAS-learning-curve.pdf}
\caption{LAS learning curve for syntactic parser according to quantity of training data. Similar shape is obtained for UAS and UPOS.}
\label{t:syntax-learning-curve}
\end{figure}

Finally, Figure~\ref{t:syntax-learning-curve} shows the learning curve when reducing the training data available to the syntactic parser. For this, we randomly sampled 10 subsets of the training data at the recording level in order to fit a target ratio from 2.5\% to 100\%. The figure shows that LAS is always better for \textbf{ORAL} representations and that \textbf{MIX} is closer to \textbf{FBU} when less data is available.
\end{comment}

% OOV results table, to address reviewer concern
% Minimal version compared to BigScience paper, to save space
\begin{table}[htb]
\centering
%\caption{Syntactic parsing performance on OOV words according to automatic transcription system. The $\Delta$ column contains the difference between the global accuracy and the accuracy on OOVs only.}
\caption{Differences in morphosyntactic performances, when parsing models of Table~\ref{t:syntax-main} are evaluated only on OOV words (OOV according to the automatic transcription system used to generate the text our LMs were trained on).}
\begin{tabular}{lrrr} \toprule									
{\bf Model} & {\bf $\Delta$LAS} & {\bf $\Delta$UAS} & {\bf $\Delta$UPOS} \\ \midrule
FBU	& -11.45 & -6.82 & -14.36 \\
MIX	& -11.93 & -7.33 & -14.07 \\
ORAL & {\bf -13.97} & {\bf -8.11} & {\bf -16.55} \\ \bottomrule
\end{tabular}
\label{t:syntax-oov}
\end{table}

%\subsection{Takeaways}
%Overall, it seems that exploiting ASR transcripts for learning LMs is slightly beneficial for syntactic parsing of speech transcripts. Some analyses presented here also show that punctuation plays an important role in representations. 
%\laurent{Please check what follows}
Finally, in Table~\ref{t:syntax-oov} we compare the drop in parsing performance between three models, when they are evaluated only against OOV words (according to the ASR system).
Revealing that the \textbf{ORAL} model variants are more affected than the off-the-shelf FlauBERT baseline (\textbf{FBU}), despite their overall better performance (as seen in Table~\ref{t:syntax-main}).
This suggests future improvements of LMs trained on ASR-generated text if ASR output tokens were more consistent with LM tokens, and also suggests applying open vocabulary ASR.

%Finally, an analysis (not reported here) of parsing performance on OOV words (according to the ASR system) reveals  that the \textbf{ORAL} model variants are more affected than the off-the-shelf FlauBERT baseline (\textbf{FBU}), despite their overall better performance. This suggests future improvements of LMs trained on ASR-generated text if ASR output tokens were more consistent with LM tokens, and also suggests applying open vocabulary ASR.

%and that 
%simulating with in text-only LMs is important at least for syntactic parsing, and that accounting for a large context is also necessary for obtaining reasonable performance. 
%In order to obtain versatile LMs that work on both text and speech, one will have to tackle those problems, for example through data augmentation or specific pre-training tasks. One area that grants more exploration is the status of speech-specific phenomena such as disfluencies that we will attend to in future work.
